Extending the Chemical Reach of the H3 Survey: Detailed Abundances of the Dwarf-galaxy Stellar Stream Wukong/LMS-1

We present the first detailed chemical-abundance analysis of stars from the dwarf-galaxy stellar stream Wukong/LMS-1 covering a wide metallicity range ($-3.5 < \rm[Fe/H] \lesssim -1.3$). We find abundance patterns that are effectively indistinguishable from the bulk of Indus and Jhelum, a pair of smaller stellar streams proposed to be dynamically associated with Wukong/LMS-1. We confirmed a carbon-enhanced metal-poor star ($\rm[C/Fe] > +0.7$ and $\rm[Fe/H] \sim -2.9$) in Wukong/LMS-1 with strong enhancements in Sr, Y, and Zr, which is peculiar given its solar-level [Ba/Fe]. Wukong/LMS-1 stars have high abundances of $\alpha$ elements up to $\rm[Fe/H] \gtrsim -2$, which is expected for relatively massive dwarfs. Towards the high-metallicity end, Wukong/LMS-1 becomes $\alpha$-poor, revealing that it probably experienced fairly standard chemical evolution. We identified a pair of N- and Na-rich stars in Wukong/LMS-1, reminiscent of multiple populations in globular clusters. This indicates that this dwarf galaxy contained at least one globular cluster that was completely disrupted in addition to two intact ones previously known to be associated with Wukong/LMS-1, which is possibly connected to similar evidence found in Indus. From these $\geq$3 globular clusters, we estimate the total mass of Wukong/LMS-1 to be ${\approx}10^{10} M_\odot$, representing ${\sim}1$% of the present-day Milky Way. Finally, the [Eu/Mg] ratio in Wukong/LMS-1 continuously increases with metallicity, making this the first example of a dwarf galaxy where the production of $r$-process elements is clearly dominated by delayed sources, presumably neutron-star mergers.

==> abundtab.tex <==
\begin{deluxetable}{lccrrrrr}
% \startlongtable
\centering
\tablewidth{\linewidth}
\tablecolumns{8}
\tabletypesize{\scriptsize}
\tablecaption{\label{tab:abunds}Stellar Abundances}
\tablehead{El. & $N$ & ul & $\log \epsilon$ & [X/H] & $\sigma_{\text{[X/H]}}$ & [X/Fe] & $\sigma_{\text{[X/Fe]}}$}
\startdata
\hline\multicolumn{8}{c}{Gaia DR3 1765600930139450752 }\\\hline
C-H   &   2 &     &$+6.12$&$-2.31$&  0.15 &$-0.07$&  0.14 \\
C-N   &   1 & $<$ &$+6.08$&$-1.75$&\nodata&$+0.49$&\nodata\\
O I   &   1 &     &$+6.98$&$-1.71$&  0.13 &$+0.54$&  0.12 \\
Na I  &   4 &     &$+4.01$&$-2.23$&  0.16 &$+0.02$&  0.16 \\
Na NLTE & & & $+3.88$&$-2.36$&&$-0.12$&\\
Mg I  &   2 &     &$+5.84$&$-1.75$&  0.08 &$+0.49$&  0.08 \\
Al I  &   2 &     &$+3.72$&$-2.73$&  0.33 &$-0.48$&  0.33 \\
Si I  &   6 &     &$+5.79$&$-1.72$&  0.07 &$+0.53$&  0.07 \\
K I   &   2 &     &$+3.54$&$-1.49$&  0.11 &$+0.76$&  0.11 \\
Ca I  &  12 &     &$+4.49$&$-1.85$&  0.08 &$+0.40$&  0.08 \\
Sc II &   7 &     &$+0.85$&$-2.30$&  0.08 &$-0.04$&  0.05 \\
Ti I  &  28 &     &$+2.92$&$-2.03$&  0.10 &$+0.22$&  0.10 \\
Ti II &  24 &     &$+2.91$&$-2.04$&  0.09 &$+0.22$&  0.05 \\
V I   &   2 &     &$+1.43$&$-2.50$&  0.06 &$-0.25$&  0.07 \\
V II  &   2 &     &$+1.73$&$-2.20$&  0.10 &$+0.06$&  0.06 \\
Cr I  &  13 &     &$+3.23$&$-2.41$&  0.13 &$-0.16$&  0.12 \\
Cr II &   5 &     &$+3.47$&$-2.17$&  0.09 &$+0.09$&  0.05 \\
Mn I  &   5 &     &$+2.75$&$-2.67$&  0.08 &$-0.43$&  0.08 \\
Fe I  &  78 &     &$+5.25$&$-2.25$&  0.04 &$+0.00$&  0.00 \\
Fe II &  19 &     &$+5.24$&$-2.26$&  0.08 &$+0.00$&  0.00 \\
Co I  &   5 &     &$+2.76$&$-2.23$&  0.12 &$+0.02$&  0.12 \\
Ni I  &  20 &     &$+3.86$&$-2.36$&  0.08 &$-0.12$&  0.08 \\
Cu I  &   1 &     &$+1.16$&$-3.03$&  0.16 &$-0.79$&  0.15 \\
Zn I  &   2 &     &$+2.41$&$-2.15$&  0.07 &$+0.10$&  0.07 \\
Sr II &   2 &     &$+0.76$&$-2.11$&  0.10 &$+0.15$&  0.10 \\
Y II  &   7 &     &$-0.33$&$-2.54$&  0.09 &$-0.28$&  0.05 \\
Zr II &   1 &     &$+0.36$&$-2.22$&  0.10 &$+0.04$&  0.05 \\
Ba II &   4 &     &$-0.17$&$-2.35$&  0.13 &$-0.10$&  0.11 \\
La II &   5 &     &$-1.10$&$-2.20$&  0.08 &$+0.06$&  0.04 \\
Eu II &   3 &     &$-1.44$&$-1.96$&  0.09 &$+0.30$&  0.06 \\
Dy II &   2 &     &$-0.79$&$-1.89$&  0.09 &$+0.37$&  0.04 \\
\hline\multicolumn{8}{c}{Gaia DR3  3573787693673899520 }\\\hline
C-H   &   2 &     &$+6.73$&$-1.70$&  0.11 &$-0.14$&  0.11 \\
C-N   &   1 & $<$ &$+7.51$&$-0.32$&\nodata&$+1.24$&\nodata\\
O I   &   1 & $<$ &$+8.86$&$+0.17$&\nodata&$+1.73$&\nodata\\
Na I  &   2 &     &$+4.87$&$-1.37$&  0.18 &$+0.19$&  0.17 \\
Na NLTE & & & $+4.34$&$-1.90$&&$-0.35$&\\
Mg I  &   2 &     &$+6.25$&$-1.35$&  0.10 &$+0.21$&  0.10 \\
Al I  &   2 &     &$+3.91$&$-2.54$&  0.23 &$-0.98$&  0.22 \\
Si I  &   4 &     &$+6.21$&$-1.30$&  0.06 &$+0.26$&  0.07 \\
K I   &   2 &     &$+4.30$&$-0.73$&  0.14 &$+0.82$&  0.13 \\
Ca I  &  12 &     &$+5.24$&$-1.10$&  0.06 &$+0.46$&  0.06 \\
Sc II &   8 &     &$+1.67$&$-1.48$&  0.08 &$+0.13$&  0.06 \\
Ti I  &  20 &     &$+3.61$&$-1.34$&  0.11 &$+0.22$&  0.10 \\
Ti II &  16 &     &$+3.73$&$-1.22$&  0.10 &$+0.40$&  0.06 \\
V I   &   2 &     &$+2.34$&$-1.59$&  0.12 &$-0.04$&  0.10 \\
V II  &   2 &     &$+2.49$&$-1.44$&  0.09 &$+0.18$&  0.07 \\
Cr I  &  10 &     &$+3.98$&$-1.66$&  0.11 &$-0.10$&  0.09 \\
Cr II &   5 &     &$+4.18$&$-1.46$&  0.09 &$+0.16$&  0.05 \\
Mn I  &   5 &     &$+3.49$&$-1.94$&  0.07 &$-0.38$&  0.07 \\
Fe I  &  80 &     &$+5.94$&$-1.56$&  0.06 &$+0.00$&  0.00 \\
Fe II &  16 &     &$+5.88$&$-1.62$&  0.09 &$+0.00$&  0.00 \\
Co I  &   3 &     &$+3.34$&$-1.65$&  0.11 &$-0.09$&  0.10 \\
Ni I  &   8 &     &$+4.66$&$-1.56$&  0.09 &$-0.00$&  0.08 \\
Zn I  &   2 &     &$+3.20$&$-1.36$&  0.08 &$+0.20$&  0.08 \\
Sr II &   2 &     &$+1.52$&$-1.35$&  0.12 &$+0.26$&  0.13 \\
Y II  &   3 &     &$+0.45$&$-1.76$&  0.10 &$-0.14$&  0.08 \\
Zr II &   1 &     &$+1.29$&$-1.29$&  0.09 &$+0.33$&  0.07 \\
Ba II &   4 &     &$+0.59$&$-1.59$&  0.10 &$+0.03$&  0.08 \\
La II &   3 &     &$-0.26$&$-1.36$&  0.10 &$+0.26$&  0.09 \\
Eu II &   2 &     &$-0.65$&$-1.17$&  0.09 &$+0.44$&  0.07 \\
Dy II &   1 &     &$-0.18$&$-1.28$&  0.18 &$+0.34$&  0.18 \\
\hline\multicolumn{8}{c}{Gaia DR3  3736372993468775424 }\\\hline
C-H   &   2 &     &$+6.99$&$-1.44$&  0.15 &$+0.18$&  0.13 \\
C-N   &   1 &     &$+6.09$&$-1.74$&  0.21 &$-0.11$&  0.18 \\
O I   &   1 &     &$+7.61$&$-1.08$&  0.11 &$+0.55$&  0.11 \\
Na I  &   4 &     &$+4.66$&$-1.58$&  0.07 &$+0.05$&  0.08 \\
Na NLTE & & & $+4.62$&$-1.62$&&$+0.01$&\\
Mg I  &   4 &     &$+6.36$&$-1.24$&  0.10 &$+0.39$&  0.10 \\
Si I  &   5 &     &$+6.28$&$-1.23$&  0.06 &$+0.40$&  0.07 \\
K I   &   2 &     &$+4.44$&$-0.59$&  0.20 &$+1.04$&  0.19 \\
Ca I  &  12 &     &$+5.13$&$-1.21$&  0.10 &$+0.42$&  0.09 \\
Sc II &   7 &     &$+1.57$&$-1.58$&  0.10 &$+0.07$&  0.07 \\
Ti I  &  36 &     &$+3.61$&$-1.34$&  0.12 &$+0.29$&  0.12 \\
Ti II &  18 &     &$+3.56$&$-1.39$&  0.09 &$+0.26$&  0.07 \\
V I   &   2 &     &$+2.06$&$-1.87$&  0.13 &$-0.24$&  0.15 \\
V II  &   1 &     &$+2.62$&$-1.31$&  0.11 &$+0.34$&  0.07 \\
Cr I  &  13 &     &$+3.85$&$-1.79$&  0.17 &$-0.16$&  0.15 \\
Cr II &   3 &     &$+4.09$&$-1.55$&  0.10 &$+0.10$&  0.06 \\
Mn I  &   5 &     &$+3.40$&$-2.04$&  0.09 &$-0.41$&  0.09 \\
Fe I  &  77 &     &$+5.87$&$-1.63$&  0.07 &$+0.00$&  0.00 \\
Fe II &  21 &     &$+5.85$&$-1.65$&  0.10 &$+0.00$&  0.00 \\
Co I  &   5 &     &$+3.37$&$-1.62$&  0.16 &$+0.01$&  0.16 \\
Ni I  &  22 &     &$+4.44$&$-1.78$&  0.11 &$-0.15$&  0.10 \\
Cu I  &   1 &     &$+2.28$&$-1.91$&  0.16 &$-0.29$&  0.14 \\
Zn I  &   2 &     &$+3.03$&$-1.53$&  0.10 &$+0.10$&  0.11 \\
Sr II &   2 &     &$+1.59$&$-1.28$&  0.05 &$+0.37$&  0.09 \\
Y II  &   6 &     &$+0.77$&$-1.44$&  0.10 &$+0.21$&  0.08 \\
Zr II &   1 &     &$+1.26$&$-1.32$&  0.18 &$+0.33$&  0.14 \\
Ba II &   4 &     &$+1.23$&$-0.95$&  0.09 &$+0.70$&  0.12 \\
La II &   5 &     &$+0.11$&$-0.99$&  0.10 &$+0.66$&  0.07 \\
Eu II &   3 &     &$-0.55$&$-1.07$&  0.08 &$+0.58$&  0.07 \\
Dy II &   3 &     &$+0.31$&$-0.79$&  0.09 &$+0.86$&  0.07 \\
\hline\multicolumn{8}{c}{Gaia DR3  3793377208170393984 }\\\hline
C-H   &   2 &     &$+6.41$&$-2.02$&  0.15 &$-0.32$&  0.14 \\
C-N   &   1 & $<$ &$+7.63$&$-0.20$&\nodata&$+1.50$&\nodata\\
O I   &   1 & $<$ &$+8.06$&$-0.63$&\nodata&$+1.07$&\nodata\\
Mg I  &   2 &     &$+6.17$&$-1.43$&  0.07 &$+0.27$&  0.07 \\
Al I  &   2 &     &$+3.72$&$-2.73$&  0.07 &$-1.03$&  0.09 \\
Si I  &   2 &     &$+6.31$&$-1.20$&  0.12 &$+0.50$&  0.11 \\
K I   &   2 &     &$+4.12$&$-0.91$&  0.12 &$+0.79$&  0.12 \\
Ca I  &  10 &     &$+5.05$&$-1.29$&  0.08 &$+0.41$&  0.08 \\
Sc II &   8 &     &$+1.61$&$-1.54$&  0.09 &$+0.14$&  0.08 \\
Ti I  &  10 &     &$+3.52$&$-1.43$&  0.12 &$+0.27$&  0.11 \\
Ti II &  14 &     &$+3.47$&$-1.48$&  0.11 &$+0.20$&  0.06 \\
V I   &   2 &     &$+2.17$&$-1.76$&  0.13 &$-0.06$&  0.12 \\
V II  &   2 &     &$+2.36$&$-1.57$&  0.11 &$+0.11$&  0.07 \\
Cr I  &   9 &     &$+3.75$&$-1.89$&  0.12 &$-0.19$&  0.11 \\
Cr II &   4 &     &$+3.91$&$-1.73$&  0.10 &$-0.05$&  0.06 \\
Mn I  &   5 &     &$+3.44$&$-1.99$&  0.07 &$-0.29$&  0.07 \\
Fe I  &  68 &     &$+5.80$&$-1.70$&  0.06 &$+0.00$&  0.00 \\
Fe II &  17 &     &$+5.82$&$-1.68$&  0.10 &$+0.00$&  0.00 \\
Co I  &   4 &     &$+3.37$&$-1.62$&  0.16 &$+0.08$&  0.15 \\
Ni I  &  12 &     &$+4.50$&$-1.72$&  0.10 &$-0.02$&  0.09 \\
Zn I  &   2 &     &$+2.91$&$-1.65$&  0.09 &$+0.05$&  0.08 \\
Sr II &   2 &     &$+1.34$&$-1.53$&  0.16 &$+0.15$&  0.14 \\
Y II  &   7 &     &$+0.36$&$-1.85$&  0.09 &$-0.17$&  0.08 \\
Zr II &   1 &     &$+0.96$&$-1.62$&  0.10 &$+0.06$&  0.06 \\
Ba II &   4 &     &$+0.56$&$-1.62$&  0.10 &$+0.06$&  0.10 \\
La II &   5 &     &$-0.39$&$-1.49$&  0.10 &$+0.19$&  0.07 \\
Eu II &   2 &     &$-0.59$&$-1.11$&  0.12 &$+0.57$&  0.07 \\
Dy II &   2 &     &$+0.17$&$-0.93$&  0.12 &$+0.75$&  0.09 \\
\hline\multicolumn{8}{c}{Gaia DR3  3891712266823336192 }\\\hline
C-H   &   2 &     &$+6.49$&$-1.94$&  0.17 &$-0.43$&  0.18 \\
C-N   &   1 &     &$+6.70$&$-1.13$&  0.28 &$+0.39$&  0.27 \\
O I   &   1 &     &$+7.67$&$-1.02$&  0.13 &$+0.49$&  0.16 \\
Na I  &   4 &     &$+4.62$&$-1.62$&  0.11 &$-0.11$&  0.12 \\
Na NLTE & & & $+4.56$&$-1.68$&&$-0.16$&\\
Mg I  &   2 &     &$+6.40$&$-1.20$&  0.12 &$+0.32$&  0.11 \\
Si I  &   4 &     &$+6.41$&$-1.10$&  0.07 &$+0.41$&  0.09 \\
K I   &   2 &     &$+4.50$&$-0.53$&  0.24 &$+0.99$&  0.23 \\
Ca I  &  10 &     &$+5.12$&$-1.22$&  0.13 &$+0.30$&  0.13 \\
Sc II &   4 &     &$+1.71$&$-1.44$&  0.14 &$+0.09$&  0.10 \\
Ti I  &  31 &     &$+3.60$&$-1.34$&  0.12 &$+0.17$&  0.12 \\
Ti II &  17 &     &$+3.59$&$-1.36$&  0.14 &$+0.17$&  0.10 \\
V I   &   2 &     &$+2.13$&$-1.80$&  0.16 &$-0.28$&  0.15 \\
V II  &   2 &     &$+2.42$&$-1.50$&  0.13 &$+0.03$&  0.10 \\
Cr I  &  12 &     &$+3.83$&$-1.80$&  0.21 &$-0.29$&  0.19 \\
Cr II &   5 &     &$+4.12$&$-1.52$&  0.13 &$+0.01$&  0.09 \\
Mn I  &   5 &     &$+3.48$&$-1.95$&  0.10 &$-0.44$&  0.10 \\
Fe I  &  76 &     &$+5.98$&$-1.52$&  0.08 &$+0.00$&  0.00 \\
Fe II &  20 &     &$+5.97$&$-1.53$&  0.12 &$+0.00$&  0.00 \\
Co I  &   5 &     &$+3.57$&$-1.42$&  0.15 &$+0.10$&  0.16 \\
Ni I  &  19 &     &$+4.53$&$-1.69$&  0.12 &$-0.17$&  0.12 \\
Cu I  &   1 &     &$+2.35$&$-1.84$&  0.20 &$-0.33$&  0.19 \\
Zn I  &   2 &     &$+3.08$&$-1.48$&  0.10 &$+0.04$&  0.13 \\
Sr II &   2 &     &$+1.53$&$-1.34$&  0.08 &$+0.19$&  0.10 \\
Y II  &   7 &     &$+0.62$&$-1.59$&  0.12 &$-0.06$&  0.10 \\
Zr II &   1 &     &$+1.27$&$-1.31$&  0.14 &$+0.23$&  0.11 \\
Ba II &   4 &     &$+0.78$&$-1.40$&  0.16 &$+0.13$&  0.15 \\
La II &   5 &     &$-0.06$&$-1.16$&  0.12 &$+0.37$&  0.08 \\
Eu II &   3 &     &$-0.40$&$-0.92$&  0.09 &$+0.62$&  0.08 \\
Dy II &   3 &     &$+0.21$&$-0.89$&  0.09 &$+0.65$&  0.11 \\
\hline\multicolumn{8}{c}{Gaia DR3  3913243629368310912 }\\\hline
C-H   &   2 &     &$+6.73$&$-1.70$&  0.17 &$-0.22$&  0.18 \\
C-N   &   1 &     &$+6.52$&$-1.31$&  0.25 &$+0.17$&  0.25 \\
O I   &   1 & $<$ &$+7.84$&$-0.84$&\nodata&$+0.64$&\nodata\\
Na I  &   4 &     &$+4.92$&$-1.32$&  0.11 &$+0.16$&  0.11 \\
Na NLTE & & & $+4.84$&$-1.40$&&$+0.08$&\\
Mg I  &   3 &     &$+6.48$&$-1.12$&  0.14 &$+0.36$&  0.13 \\
Si I  &   4 &     &$+6.69$&$-0.82$&  0.06 &$+0.66$&  0.08 \\
K I   &   2 &     &$+4.33$&$-0.70$&  0.21 &$+0.78$&  0.20 \\
Ca I  &  12 &     &$+5.36$&$-0.98$&  0.13 &$+0.50$&  0.13 \\
Sc II &   6 &     &$+1.90$&$-1.25$&  0.09 &$+0.32$&  0.11 \\
Ti I  &  26 &     &$+3.88$&$-1.07$&  0.14 &$+0.41$&  0.14 \\
Ti II &  18 &     &$+3.77$&$-1.18$&  0.12 &$+0.38$&  0.08 \\
V I   &   2 &     &$+2.31$&$-1.62$&  0.19 &$-0.14$&  0.18 \\
Cr I  &  14 &     &$+4.09$&$-1.55$&  0.21 &$-0.07$&  0.20 \\
Cr II &   2 &     &$+4.32$&$-1.32$&  0.18 &$+0.25$&  0.14 \\
Mn I  &   5 &     &$+3.66$&$-1.77$&  0.11 &$-0.28$&  0.11 \\
Fe I  &  61 &     &$+6.02$&$-1.48$&  0.06 &$+0.00$&  0.00 \\
Fe II &  20 &     &$+5.94$&$-1.56$&  0.13 &$+0.00$&  0.00 \\
Co I  &   5 &     &$+3.60$&$-1.39$&  0.19 &$+0.09$&  0.19 \\
Ni I  &  20 &     &$+4.64$&$-1.58$&  0.14 &$-0.10$&  0.14 \\
Cu I  &   1 &     &$+2.39$&$-1.80$&  0.19 &$-0.32$&  0.18 \\
Zn I  &   2 &     &$+3.20$&$-1.36$&  0.11 &$+0.12$&  0.13 \\
Sr II &   2 &     &$+1.61$&$-1.26$&  0.13 &$+0.30$&  0.15 \\
Y II  &   7 &     &$+0.59$&$-1.62$&  0.10 &$-0.06$&  0.10 \\
Zr II &   1 &     &$+1.16$&$-1.42$&  0.14 &$+0.14$&  0.10 \\
Ba II &   4 &     &$+0.62$&$-1.56$&  0.13 &$-0.00$&  0.12 \\
La II &   4 &     &$+0.05$&$-1.05$&  0.12 &$+0.51$&  0.10 \\
Eu II &   3 &     &$-0.32$&$-0.84$&  0.09 &$+0.72$&  0.08 \\
Dy II &   3 &     &$+0.28$&$-0.82$&  0.06 &$+0.74$&  0.11 \\
\hline\multicolumn{8}{c}{Gaia DR3  3939346894405032576 }\\\hline
C-H   &   2 &     &$+6.80$&$-1.63$&  0.17 &$+0.01$&  0.15 \\
C-N   &   1 & $<$ &$+7.56$&$-0.27$&\nodata&$+1.37$&\nodata\\
O I   &   1 & $<$ &$+8.62$&$-0.07$&\nodata&$+1.57$&\nodata\\
Na I  &   2 &     &$+4.89$&$-1.35$&  0.21 &$+0.29$&  0.18 \\
Na NLTE & & & $+4.32$&$-1.92$&&$-0.28$&\\
Mg I  &   2 &     &$+6.40$&$-1.20$&  0.10 &$+0.44$&  0.10 \\
Al I  &   2 &     &$+3.79$&$-2.66$&  0.15 &$-1.02$&  0.13 \\
Si I  &   1 &     &$+6.27$&$-1.24$&  0.21 &$+0.40$&  0.17 \\
K I   &   2 &     &$+4.33$&$-0.70$&  0.20 &$+0.95$&  0.19 \\
Ca I  &   8 &     &$+5.22$&$-1.12$&  0.09 &$+0.53$&  0.09 \\
Sc II &   6 &     &$+1.65$&$-1.50$&  0.10 &$+0.17$&  0.06 \\
Ti I  &   9 &     &$+3.81$&$-1.14$&  0.15 &$+0.50$&  0.13 \\
Ti II &  13 &     &$+3.74$&$-1.21$&  0.11 &$+0.47$&  0.07 \\
V I   &   1 &     &$+2.55$&$-1.38$&  0.11 &$+0.27$&  0.10 \\
V II  &   2 &     &$+2.55$&$-1.38$&  0.11 &$+0.29$&  0.10 \\
Cr I  &   4 &     &$+3.91$&$-1.73$&  0.16 &$-0.09$&  0.13 \\
Cr II &   3 &     &$+4.04$&$-1.60$&  0.09 &$+0.07$&  0.04 \\
Mn I  &   5 &     &$+3.62$&$-1.81$&  0.10 &$-0.17$&  0.09 \\
Fe I  &  51 &     &$+5.86$&$-1.64$&  0.08 &$+0.00$&  0.00 \\
Fe II &  11 &     &$+5.83$&$-1.67$&  0.09 &$+0.00$&  0.00 \\
Co I  &   4 &     &$+3.34$&$-1.65$&  0.12 &$-0.01$&  0.11 \\
Ni I  &   7 &     &$+4.59$&$-1.63$&  0.10 &$+0.01$&  0.09 \\
Zn I  &   2 &     &$+3.03$&$-1.53$&  0.11 &$+0.11$&  0.10 \\
Sr II &   2 &     &$+1.27$&$-1.60$&  0.21 &$+0.08$&  0.19 \\
Y II  &   3 &     &$+0.69$&$-1.52$&  0.11 &$+0.15$&  0.08 \\
Ba II &   3 &     &$+0.61$&$-1.57$&  0.13 &$+0.10$&  0.10 \\
La II &   1 &     &$-0.11$&$-1.21$&  0.16 &$+0.46$&  0.14 \\
Eu II &   2 &     &$-0.52$&$-1.04$&  0.11 &$+0.64$&  0.08 \\
Dy II &   1 &     &$+0.20$&$-0.91$&  0.17 &$+0.77$&  0.16 \\
\enddata
\tablecomments{The ``ul'' column is an upper limit flag.}
\end{deluxetable}

\newpage
